Beyond Fine-tuning: Few-Sample Sentence Embedding Transfer

Fine-tuning (FT) pre-trained sentence embedding models on small datasets has been shown to have limitations. In this paper we show that concatenating the embeddings from the pre-trained model with those from a simple sentence embedding model trained only on the target data, can improve over the performance of FT for few-sample tasks. To this end, a linear classifier is trained on the combined embeddings, either by freezing the embedding model weights or training the classifier and embedding models end-to-end. We perform evaluation on seven small datasets from NLP tasks and show that our approach with end-to-end training outperforms FT with negligible computational overhead. Further, we also show that sophisticated combination techniques like CCA and KCCA do not work as well in practice as concatenation. We provide theoretical analysis to explain this empirical observation.

==> AACL-IJCNLP Camera Ready#168/small_dataset_full_table.tex <==
\begin{table*}[ht]
\centering
\resizebox{2\columnwidth}{!}{
\begin{tabular}{cccc|c|c|c|c|}
\cline{5-8}
&       &      &        & \textbf{BOW }         & \textbf{{\CNNR}}      & \textbf{{\CNNS}}    & \textbf{{\CNNNS}} \\ \hline
\multicolumn{1}{|c|}{\multirow{11}{*}{\textbf{Amazon} }} & \multicolumn{3}{c|}{\textbf{Default}}                                                                                  &        79.20 $\pm$ 2.31      & 91.10 $\pm$ 1.64   & 94.70 $\pm$ 0.64   & 95.90 $\pm$ 0.70    \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{BERT}}}      & \multicolumn{1}{c|}{\multirow{3}{*}{94.00 $\pm$ 0.02}} & {\CATEE} & - & 94.05 $\pm$ 0.23  & 95.70 $\pm$ 0.50  & \emph{\textbf{96.75 $\pm$ 0.76}} \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\CATFr} & 89.59 $\pm$ 1.22 & 93.20 $\pm$ 0.98  & 95.30 $\pm$ 0.46  & 96.40 $\pm$ 1.11   \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\KCCAFr}   & 89.12 $\pm$ 0.47 & 91.50 $\pm$ 1.63  & 94.30 $\pm$ 0.46  & 95.80 $\pm$ 0.40   \\ \cline{4-8}
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\CCAFr}    & 50.91 $\pm$ 1.12 & 79.10 $\pm$ 2.51  & 83.60 $\pm$ 1.69  & 81.30 $\pm$ 3.16   \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{GenSen}}}    & \multicolumn{1}{c|}{\multirow{3}{*}{82.55 $\pm$ 0.82}} & {\CATFr} & 82.82 $\pm$ 0.97 & 92.80 $\pm$ 1.25  & 94.10 $\pm$ 0.70  & 95.00 $\pm$ 1.0    \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\KCCAFr}   & 79.21 $\pm$ 2.28 & 91.30 $\pm$ 1.42  & 94.80 $\pm$ 0.75  & \textbf{ 95.90 $\pm$ 0.30}   \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\CCAFr}    & 52.80 $\pm$ 0.74  & 80.60 $\pm$ 4.87 & 83.00 $\pm$ 2.45  & 84.95 $\pm$ 1.45   \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{InferSent}}} & \multicolumn{1}{c|}{\multirow{3}{*}{85.29 $\pm$ 1.61}} & {\CATFr} & 51.89 $\pm$ 0.62 & 90.30 $\pm$ 1.48 & 94.70 $\pm$ 1.10 & 95.90 $\pm$ 0.70  \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\KCCAFr}   & 52.29 $\pm$ 0.74 & 91.70 $\pm$ 1.49 & 95.00 $\pm$ 0.00 & \textbf{ 96.00 $\pm$ 0.00 } \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\CCAFr}    & 53.10 $\pm$ 0.82  & 61.10 $\pm$ 3.47 & 65.50 $\pm$ 3.69 & 71.40 $\pm$ 3.04   \\ \hline
\multicolumn{1}{|c|}{\multirow{11}{*}{\textbf{Yelp}}}   & \multicolumn{3}{c|}{\textbf{Default}}                                                                                  &         $81.3 \pm 2.72$     & 92.71$\pm$ 0.46  & 95.25 $\pm$ 0.39 & 95.83 $\pm$ 0.14  \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{BERT}}}      & \multicolumn{1}{c|}{\multirow{3}{*}{91.67 $\pm$ 0.00}} & {\CATEE} & - & 96.23 $\pm$ 1.04  & 97.23 $\pm$ 0.70  &  \emph{\textbf{98.34 $\pm$ 0.62}}  \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                         &      {\CATFr} & 89.03 $\pm$ 0.70 & 96.50 $\pm$ 1.33  & 97.10 $\pm$ 0.70  & 98.30 $\pm$ 0.78  \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\KCCAFr}   & 88.51 $\pm$ 1.22 & 91.54 $\pm$ 4.63 & 91.91 $\pm$1.13  & 96.2 $\pm$ 0.87   \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\CCAFr}    & 50.27 $\pm$ 1.33 & 71.53 $\pm$ 2.46 & 67.83 $\pm$ 3.07 & 69.4 $\pm$ 3.35   \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{GenSen}}}    & \multicolumn{1}{c|}{\multirow{3}{*}{86.75 $\pm$ 0.79}} & {\CATFr} & 85.94 $\pm$ 1.04 & 94.24 $\pm$ 0.53 & 95.77 $\pm$ 0.36 & \textbf{ 96.03 $\pm$ 0.23 } \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\KCCAFr}   & 83.35 $\pm$ 1.79 & 92.58 $\pm$ 0.31 & 95.41 $\pm$ 0.45 & 95.06 $\pm$ 0.56  \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\CCAFr}    & 57.14 $\pm$ 0.84 & 84.27 $\pm$ 1.68 & 86.94 $\pm$ 1.62 & 87.27$\pm$ 1.81   \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{InferSent}}} & \multicolumn{1}{c|}{\multirow{3}{*}{85.7 $\pm$ 1.12}}  & {\CATFr} & 50.83 $\pm$ 0.42 & 91.94 $\pm$ 0.46  & 96.10 $\pm$ 1.30 & \textbf{ 97.00 $\pm$ 0.77 } \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\KCCAFr}   & 50.80 $\pm$ 0.65  & 91.13 $\pm$ 1.63  & 95.45 $\pm$ 0.23  & 95.57 $\pm$ 0.55   \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\CCAFr}    & 55.91 $\pm$ 1.23 & 60.80 $\pm$ 2.22 & 54.70 $\pm$ 1.34  & 59.50 $\pm$ 1.85   \\ \hline
\multicolumn{1}{|c|}{\multirow{11}{*}{\textbf{IMDB}}}   & \multicolumn{3}{c|}{\textbf{Default}}                                                                                  &          $89.30 \pm 1.00$    & 93.25 $\pm$ 0.38 & 96.62 $\pm$ 0.46 & 96.76 $\pm$ 0.26  \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{BERT}}}      & \multicolumn{1}{c|}{\multirow{3}{*}{92.33 $\pm$ 0.00}} & {\CATEE} & -  & 97.07 $\pm$ 0.95  &  98.31 $\pm$ 0.83   & \emph{\textbf{98.42 $\pm$ 0.78 } }  \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                         &  {\CATFr} & 89.27 $\pm$ 0.97 & 96.20 $\pm$ 2.18  & 98.10 $\pm$ 0.94  & 98.30 $\pm$ 1.35  \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\KCCAFr}   & 88.29 $\pm$ 0.65 & 94.10 $\pm$ 1.87  & 97.90 $\pm$ 0.30  & 97.20 $\pm$ 0.40  \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\CCAFr}    & 51.03 $\pm$ 1.20 & 80.80 $\pm$ 2.75  & 83.30 $\pm$ 4.47  & 84.97 $\pm$ 1.44   \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{GenSen}}}    & \multicolumn{1}{c|}{\multirow{3}{*}{86.41 $\pm$ 0.66}} & {\CATFr} & 86.86 $\pm$ 0.62 & 95.63 $\pm$ 0.47 & 97.22 $\pm$ 0.27 & \textbf{ 97.42 $\pm$ 0.31 } \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\KCCAFr}   & 84.72 $\pm$ 0.93 & 93.23 $\pm$ 0.38 & 96.19 $\pm$ 0.21 & 96.60 $\pm$ 0.37  \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\CCAFr}    & 51.48 $\pm$ 1.02 & 86.28 $\pm$ 1.76 & 87.30 $\pm$ 2.12 & 87.47 $\pm$ 2.17  \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{InferSent}}} & \multicolumn{1}{c|}{\multirow{3}{*}{84.3 $\pm$ 0.63}}  & {\CATFr} & 50.36 $\pm$ 0.62 & 92.30 $\pm$ 1.26 & 97.90 $\pm$ 1.37 & 97.10 $\pm$ 1.22  \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\KCCAFr}   & 50.09 $\pm$ 0.68 & 92.40 $\pm$ 1.11 & 97.62 $\pm$0.48  & \textbf{ 98.20 $\pm$ 1.40}  \\ \cline{4-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                              & {\CCAFr}    & 52.56 $\pm$ 1.15 & 54.50 $\pm$ 4.92  & 54.20 $\pm$ 5.15 & 61.00 $\pm$ 4.64  \\ \hline
\end{tabular}}
\caption{Test accuracy ( $\pm$ std dev)  for Amazon, Yelp and IMDB review datasets. Default values are performance of the domain specific models. Default values for BERT, Gensen and InferSent correspond to fine-tuning them. Best results for each pre-trained model are highlighted in boldface.}
\label{tab:small_datasets_full}
\end{table*}

